Towards Effective Semantic OOD Detection in Unseen Domains: A Domain Generalization Perspective

Two prevalent types of distributional shifts in machine learning are the covariate shift (as observed across different domains) and the semantic shift (as seen across different classes). Traditional OOD detection techniques typically address only one of these shifts. However, real-world testing environments often present a combination of both covariate and semantic shifts. In this study, we introduce a novel problem, semantic OOD detection across domains, which simultaneously addresses both distributional shifts. To this end, we introduce two regularization strategies: domain generalization regularization, which ensures semantic invariance across domains to counteract the covariate shift, and OOD detection regularization, designed to enhance OOD detection capabilities against the semantic shift through energy bounding. Through rigorous testing on three standard domain generalization benchmarks, our proposed framework showcases its superiority over conventional domain generalization approaches in terms of OOD detection performance. Moreover, it holds its ground by maintaining comparable InD classification accuracy.

==> references.tex <==
@book{em:86,
  editor  = "Engelmore, Robert and Morgan, Anthony",
  title   = "Blackboard Systems",
  year    = 1986,
  address = "Reading, Mass.",
  publisher = "Addison-Wesley",
}

@inproceedings{c:83,
  author  = "Clancey, William J.",
  year    = 1983,
  title   = "{Communication, Simulation, and Intelligent
Agents: Implications of Personal Intelligent Machines
for Medical Education}",
  booktitle="Proceedings of the Eighth International Joint Conference on Artificial Intelligence {(IJCAI-83)}", 
  pages   = "556-560",
  address = "Menlo Park, Calif",
  publisher = "{IJCAI Organization}",
}
@inproceedings{c:84,
  author  = "Clancey, William J.",
  year    = 1984,
  title   = "{Classification Problem Solving}",
  booktitle = "Proceedings of the Fourth National 
              Conference on Artificial Intelligence",
  pages   = "45-54",
  address = "Menlo Park, Calif.",
  publisher="AAAI Press",
}
@article{r:80,
  author = {Robinson, Arthur L.},
  title = {New Ways to Make Microcircuits Smaller},
  volume = {208},
  number = {4447},
  pages = {1019--1022},
  year = {1980},
  doi = {10.1126/science.208.4447.1019},
  publisher = {American Association for the Advancement of Science},
  issn = {0036-8075},
  URL = {https://science.sciencemag.org/content/208/4447/1019},
  eprint = {https://science.sciencemag.org/content/208/4447/1019.full.pdf},
  journal = {Science},
}
@article{r:80x,
  author  = "Robinson, Arthur L.",
  year    = 1980,
  title   = "{New Ways to Make Microcircuits Smaller---Duplicate Entry}",
  journal = "Science",
  volume  =  208,
  pages   = "1019-1026",
}
@article{hcr:83,
title = {Strategic explanations for a diagnostic consultation system},
journal = {International Journal of Man-Machine Studies},
volume = {20},
number = {1},
pages = {3-19},
year = {1984},
issn = {0020-7373},
doi = {https://doi.org/10.1016/S0020-7373(84)80003-6},
url = {https://www.sciencedirect.com/science/article/pii/S0020737384800036},
author = {Diane Warner Hasling and William J. Clancey and Glenn Rennels},
abstract = {This article examines the problem of automatte explanation of reasoning, especially as it relates to expert systems. By explanation we mean the ability of a program to discuss what it is doing in some understandable way. We first present a general framework in which to view explanation and review some of the research done in this area. We then focus on the explanation system for NEOMYCIN, a medical consultation program. A consultation program interactively helps a user to solve a problem. Our goal is to have NEOMYCIN explain its problem-solving strategies. An explanation of strategy describes the plan the program is using to reach a solution. Such an explanation is usually concrete, referring to aspects of the current problem situation. Abstract explanations articulate a general principle, which can be applied in different situations; such explanations are useful in teaching and in explaining by analogy. We describe the aspects of NEOMYCIN that make abstract strategic explanations possible—the representation of strategic knowledge explicitly and separately from domain knowledge— and demonstrate how this representation can be used to generate explanations.}
}
@article{hcrt:83,
  author  = "Hasling, Diane Warner and Clancey, William J. and Rennels, Glenn R. and Test, Thomas",
  year    = 1983,
  title   = "{Strategic Explanations in Consultation---Duplicate}",
  journal = "The International Journal of Man-Machine Studies",
  volume  = 20,
  number  = 1,
  pages   = "3-19",
}
@techreport{r:86,
  author  = "Rice, James",
  year    = 1986,
  title   = "{Poligon: A System for Parallel Problem Solving}",
  type    = "Technical Report", 
  number  = "KSL-86-19", 
  institution = "Dept.\ of Computer Science, Stanford Univ.",
}
@phdthesis{c:79,
  author  = "Clancey, William J.",
  year    = 1979,
  title   = "{Transfer of Rule-Based Expertise
through a Tutorial Dialogue}",
  type    = "{Ph.D.} diss.",
  school  = "Dept.\ of Computer Science, Stanford Univ.",
  address = "Stanford, Calif.",
}
@unpublished{c:21,
  author  = "Clancey, William J.",
  title   = "{The Engineering of Qualitative Models}",
  year    = 2021,
  note    = "Forthcoming",
}
@misc{c:22,
      title={Attention Is All You Need}, 
      author={Ashish Vaswani and Noam Shazeer and Niki Parmar and Jakob Uszkoreit and Llion Jones and Aidan N. Gomez and Lukasz Kaiser and Illia Polosukhin},
      year={2017},
      eprint={1706.03762},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}
@misc{c:23,
  title        = "Pluto: The 'Other' Red Planet",
  author       = "{NASA}",
  howpublished = "\url{https://www.nasa.gov/nh/pluto-the-other-red-planet}",
  year         = 2015,
  note         = "Accessed: 2018-12-06"
}
@article{hendrycks2016baseline,
  title={A baseline for detecting misclassified and out-of-distribution examples in neural networks},
  author={Hendrycks, Dan and Gimpel, Kevin},
  journal={arXiv preprint arXiv:1610.02136},
  year={2016}
}
@article{liu2020energy,
  title={Energy-based out-of-distribution detection},
  author={Liu, Weitang and Wang, Xiaoyun and Owens, John and Li, Yixuan},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={21464--21475},
  year={2020}
}
@article{mukhoti2021deep,
  title={Deep deterministic uncertainty: A simple baseline},
  author={Mukhoti, Jishnu and Kirsch, Andreas and van Amersfoort, Joost and Torr, Philip HS and Gal, Yarin},
  journal={arXiv preprint arXiv:2102.11582},
  year={2021}
}
@article{scholkopf1999support,
  title={Support vector method for novelty detection},
  author={Sch{\"o}lkopf, Bernhard and Williamson, Robert C and Smola, Alex and Shawe-Taylor, John and Platt, John},
  journal={Advances in neural information processing systems},
  volume={12},
  year={1999}
}
@inproceedings{li2017deeper,
  title={Deeper, broader and artier domain generalization},
  author={Li, Da and Yang, Yongxin and Song, Yi-Zhe and Hospedales, Timothy M},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={5542--5550},
  year={2017}
}
@inproceedings{torralba2011unbiased,
  title={Unbiased look at dataset bias},
  author={Torralba, Antonio and Efros, Alexei A},
  booktitle={CVPR 2011},
  pages={1521--1528},
  year={2011},
  organization={IEEE}
}
@article{arjovsky2019invariant,
  title={Invariant risk minimization},
  author={Arjovsky, Martin and Bottou, L{\'e}on and Gulrajani, Ishaan and Lopez-Paz, David},
  journal={arXiv preprint arXiv:1907.02893},
  year={2019}
}
@book{vapnik1999nature,
  title={The nature of statistical learning theory},
  author={Vapnik, Vladimir},
  year={1999},
  publisher={Springer science \& business media}
}
@article{yan2020improve,
  title={Improve unsupervised domain adaptation with mixup training},
  author={Yan, Shen and Song, Huan and Li, Nanxiang and Zou, Lincan and Ren, Liu},
  journal={arXiv preprint arXiv:2001.00677},
  year={2020}
}
@article{robey2021model,
  title={Model-based domain generalization},
  author={Robey, Alexander and Pappas, George J and Hassani, Hamed},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={20210--20229},
  year={2021}
}
@article{gulrajani2020search,
  title={In search of lost domain generalization},
  author={Gulrajani, Ishaan and Lopez-Paz, David},
  journal={arXiv preprint arXiv:2007.01434},
  year={2020}
}

@article{lee2017training,
  title={Training confidence-calibrated classifiers for detecting out-of-distribution samples},
  author={Lee, Kimin and Lee, Honglak and Lee, Kibok and Shin, Jinwoo},
  journal={arXiv preprint arXiv:1711.09325},
  year={2017}
}

@article{kawakami2020learning,
  title={Learning robust and multilingual speech representations},
  author={Kawakami, Kazuya and Wang, Luyu and Dyer, Chris and Blunsom, Phil and Oord, Aaron van den},
  journal={arXiv preprint arXiv:2001.11128},
  year={2020}
}

@article{grosse2017statistical,
  title={On the (statistical) detection of adversarial examples},
  author={Grosse, Kathrin and Manoharan, Praveen and Papernot, Nicolas and Backes, Michael and McDaniel, Patrick},
  journal={arXiv preprint arXiv:1702.06280},
  year={2017}
}

@inproceedings{ruff2018deep,
  title={Deep one-class classification},
  author={Ruff, Lukas and Vandermeulen, Robert and Goernitz, Nico and Deecke, Lucas and Siddiqui, Shoaib Ahmed and Binder, Alexander and M{\"u}ller, Emmanuel and Kloft, Marius},
  booktitle={International conference on machine learning},
  pages={4393--4402},
  year={2018},
  organization={PMLR}
}
@article{yang2021generalized,
  title={Generalized out-of-distribution detection: A survey},
  author={Yang, Jingkang and Zhou, Kaiyang and Li, Yixuan and Liu, Ziwei},
  journal={arXiv preprint arXiv:2110.11334},
  year={2021}
}
@article{hastie1996discriminant,
  title={Discriminant analysis by Gaussian mixtures},
  author={Hastie, Trevor and Tibshirani, Robert},
  journal={Journal of the Royal Statistical Society Series B: Statistical Methodology},
  volume={58},
  number={1},
  pages={155--176},
  year={1996},
  publisher={Oxford University Press}
}
@article{lecun2006tutorial,
  title={A tutorial on energy-based learning},
  author={LeCun, Yann and Chopra, Sumit and Hadsell, Raia and Ranzato, M and Huang, Fujie},
  journal={Predicting structured data},
  volume={1},
  number={0},
  year={2006}
}
@article{liang2017enhancing,
  title={Enhancing the reliability of out-of-distribution image detection in neural networks},
  author={Liang, Shiyu and Li, Yixuan and Srikant, Rayadurgam},
  journal={arXiv preprint arXiv:1706.02690},
  year={2017}
}
@article{lee2018simple,
  title={A simple unified framework for detecting out-of-distribution samples and adversarial attacks},
  author={Lee, Kimin and Lee, Kibok and Lee, Honglak and Shin, Jinwoo},
  journal={Advances in neural information processing systems},
  volume={31},
  year={2018}
}
@article{shama2019detecting,
  title={Detecting out-of-distribution examples with in-distribution examples and gram matrices},
  author={Shama Sastry, Chandramouli and Oore, Sageev},
  journal={arXiv e-prints},
  pages={arXiv--1912},
  year={2019}
}
@inproceedings{zhang2022towards,
  title={Towards principled disentanglement for domain generalization},
  author={Zhang, Hanlin and Zhang, Yi-Fan and Liu, Weiyang and Weller, Adrian and Sch{\"o}lkopf, Bernhard and Xing, Eric P},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={8024--8034},
  year={2022}
}
@inproceedings{li2018learning,
  title={Learning to generalize: Meta-learning for domain generalization},
  author={Li, Da and Yang, Yongxin and Song, Yi-Zhe and Hospedales, Timothy},
  booktitle={Proceedings of the AAAI conference on artificial intelligence},
  volume={32},
  number={1},
  year={2018}
}
@article{ganin2016domain,
  title={Domain-adversarial training of neural networks},
  author={Ganin, Yaroslav and Ustinova, Evgeniya and Ajakan, Hana and Germain, Pascal and Larochelle, Hugo and Laviolette, Fran{\c{c}}ois and Marchand, Mario and Lempitsky, Victor},
  journal={The journal of machine learning research},
  volume={17},
  number={1},
  pages={2096--2030},
  year={2016},
  publisher={JMLR. org}
}
@article{balaji2018metareg,
  title={Metareg: Towards domain generalization using meta-regularization},
  author={Balaji, Yogesh and Sankaranarayanan, Swami and Chellappa, Rama},
  journal={Advances in neural information processing systems},
  volume={31},
  year={2018}
}

@inproceedings{huang2018multimodal,
  title={Multimodal unsupervised image-to-image translation},
  author={Huang, Xun and Liu, Ming-Yu and Belongie, Serge and Kautz, Jan},
  booktitle={Proceedings of the European conference on computer vision (ECCV)},
  pages={172--189},
  year={2018}
}
@article{ruff2021unifying,
  title={A unifying review of deep and shallow anomaly detection},
  author={Ruff, Lukas and Kauffmann, Jacob R and Vandermeulen, Robert A and Montavon, Gr{\'e}goire and Samek, Wojciech and Kloft, Marius and Dietterich, Thomas G and M{\"u}ller, Klaus-Robert},
  journal={Proceedings of the IEEE},
  volume={109},
  number={5},
  pages={756--795},
  year={2021},
  publisher={IEEE}
}
@inproceedings{sabokrou2018adversarially,
  title={Adversarially learned one-class classifier for novelty detection},
  author={Sabokrou, Mohammad and Khalooei, Mohammad and Fathy, Mahmood and Adeli, Ehsan},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={3379--3388},
  year={2018}
}
@inproceedings{bhattacharjee2020multi,
  title={Multi-class novelty detection using mix-up technique},
  author={Bhattacharjee, Supritam and Mandal, Devraj and Biswas, Soma},
  booktitle={Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision},
  pages={1400--1409},
  year={2020}
}
@article{geng2020recent,
  title={Recent advances in open set recognition: A survey},
  author={Geng, Chuanxing and Huang, Sheng-jun and Chen, Songcan},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={43},
  number={10},
  pages={3614--3631},
  year={2020},
  publisher={IEEE}
}

@article{gui2022good,
  title={Good: A graph out-of-distribution benchmark},
  author={Gui, Shurui and Li, Xiner and Wang, Limei and Ji, Shuiwang},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={2059--2073},
  year={2022}
}

@inproceedings{ming2022impact,
  title={On the impact of spurious correlation for out-of-distribution detection},
  author={Ming, Yifei and Yin, Hang and Li, Yixuan},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={36},
  number={9},
  pages={10051--10059},
  year={2022}
}
@article{zhang2017mixup,
  title={mixup: Beyond empirical risk minimization},
  author={Zhang, Hongyi and Cisse, Moustapha and Dauphin, Yann N and Lopez-Paz, David},
  journal={arXiv preprint arXiv:1710.09412},
  year={2017}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@article{zhou2018interpreting,
  title={Interpreting deep visual representations via network dissection},
  author={Zhou, Bolei and Bau, David and Oliva, Aude and Torralba, Antonio},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={41},
  number={9},
  pages={2131--2145},
  year={2018},
  publisher={IEEE}
}

@inproceedings{rauker2023toward,
  title={Toward transparent ai: A survey on interpreting the inner structures of deep neural networks},
  author={R{\"a}uker, Tilman and Ho, Anson and Casper, Stephen and Hadfield-Menell, Dylan},
  booktitle={2023 IEEE Conference on Secure and Trustworthy Machine Learning (SaTML)},
  pages={464--483},
  year={2023},
  organization={IEEE}
}
